Instance Separation Emerges from Inpainting

Deep neural networks trained to inpaint partially occluded images show a deep understanding of image composition and have even been shown to remove objects from images convincingly. In this work, we investigate how this implicit knowledge of image composition can be leveraged for fully self-supervised instance separation. We propose a measure for the independence of two image regions given a fully self-supervised inpainting network and separate objects by maximizing this independence. We evaluate our method on two microscopy image datasets and show that it reaches similar segmentation performance to fully supervised methods.

==> authors.tex <==
\begin{icmlauthorlist}
\icmlauthor{Steffen Wolf}{iwr}
\icmlauthor{Fred A. Hamprecht}{iwr}
\icmlauthor{Jan Funke}{jan}
\end{icmlauthorlist}
\icmlaffiliation{iwr}{HCI, Heidelberg University, Germany}
\icmlaffiliation{jan}{HHMI Janelia, Ashburn, VA}
\icmlcorrespondingauthor{Steffen Wolf}{steffen.wolf@iwr.uni-heidelberg.de}
\icmlkeywords{Machine Learning, ICML, Cell Segmentation, Inpainting, Self-Supervised Learning}


==> figures/plots/iou_hela.tikz.tex <==
\begin{tikzpicture}[scale=0.8,transform shape]
  \begin{axis}[
    xlabel={IoU threshold},
    ylabel={detection accuracy},
    legend style={at={(0.02,0.02)},anchor=south west},
    xmin=0,
    xmax=1,
    width=10cm,
    height=8cm,
    ]

    \def\plotfile{figures/plots/iou_plots/Hela.csv}

    \addplot[funkey_color_1,thick,only marks,mark=*] coordinates {(0.2, 0.2)};
    \addlegendentry[funkey_color_1]{\footnotesize \ouraffs + \fgnet}
    \addplot[funkey_color_1,dotted,thick,no marks] table [
      col sep=comma,
      x=IoUthreshold,
      y=size1]
        {\plotfile};
    \addlegendentry{17 labeled instances}
    \addplot[funkey_color_1,dashed,thick,no marks] table [
      col sep=comma,
      x=IoUthreshold,
      y=size4]
        {\plotfile};
    \addlegendentry{52 labeled instances}

    \addplot[funkey_color_2,thick,only marks,mark=*] coordinates {(0.2, 0.2)};
    \addlegendentry[funkey_color_2]{\footnotesize \affnet + \fgnet}
    \addplot[funkey_color_2,dotted,thick,no marks] table [
      col sep=comma,
      x=IoUthreshold,
      y=size1_supervised_affinities]
        {\plotfile};
    \addlegendentry{17 labeled instances}
    \addplot[funkey_color_2,dashed,thick,no marks] table [
      col sep=comma,
      x=IoUthreshold,
      y=size4_supervised_affinities]
        {\plotfile};
    \addlegendentry{52 labeled instances}

    \addplot[funkey_color_3,thick,no marks] table [
      col sep=comma,
      x=IoUthreshold,
      y=unsupervised_affinities_affinities_bg_true]
        {\plotfile};
    \addlegendentry[funkey_color_3]{\ouraffs + \truefg}

    \addplot[gray,thick,no marks] table [
      col sep=comma,
      x=IoUthreshold,
      y=connected_components_bg_true]
        {\plotfile};
    \addlegendentry{CC on \truefg}

  \end{axis}
\end{tikzpicture}

